Model Based Screening Embedded Bayesian Variable Selection for Ultra-high Dimensional Settings

We develop a Bayesian variable selection method, called SVEN, based on a hierarchical Gaussian linear model with priors placed on the regression coefficients as well as on the model space. Sparsity is achieved by using degenerate spike priors on inactive variables, whereas Gaussian slab priors are placed on the coefficients for the important predictors making the posterior probability of a model available in explicit form (up to a normalizing constant). The strong model selection consistency is shown to be attained when the number of predictors grows nearly exponentially with the sample size and even when the norm of mean effects solely due to the unimportant variables diverge, which is a novel attractive feature. An appealing byproduct of SVEN is the construction of novel model weight adjusted prediction intervals. Embedding a unique model based screening and using fast Cholesky updates, SVEN produces a highly scalable computational framework to explore gigantic model spaces, rapidly identify the regions of high posterior probabilities and make fast inference and prediction. A temperature schedule guided by our model selection consistency derivations is used to further mitigate multimodal posterior distributions. The performance of SVEN is demonstrated through a number of simulation experiments and a real data example from a genome wide association study with over half a million markers.

==> 5Computation.tex <==
\section{Computation}
\subsection{The Bayesian variable selection algorithm}
To explore the model space that contains $2^p$ models, the general method is using MCMC to sample from the corresponding posterior and estimate posterior probabilities. However, in ultrahigh dimensional settings where the number of variables is allowed to grow with sample size at nearly exponential rate, MCMC chains converge at a very slow rate. In addition, due to the vast model space, MCMC sample size used in practice may not be large enough to allow the chains to visit the regions of high posterior probability over models. To conquer this problem, we propose an algorithm to find the MAP model by efficiently navigating through huge model spaces and rapidly identifying regions containing models with high posterior probabilities. The proposed algorithm also incorporates the idea of model screening which is introduce in section 4 and simulated annealing, a well known global optimization algorithm, by (\citealp{kirk:gela:1983}). 

The algorithm essentially evaluates the neighborhood of the current model ($\text{nbd}(\gamma)$) at each step and make a move to another potential model using some sampling strategy. Recall from section 4 that $\text{nbd}(\gamma)=\gamma^{+} \cup \gamma^{\circ} \cup \gamma^{-}$. At each iteration, the posterior probability of each model in $\text{nbd}(\gamma)$ is computed, and then a screening on those neighbor models is conducted so that only models with high posterior probabilities are taken into account for the next steps. To be specific, let $\bm{M}_\text{scr}$ denote the set consisting of the models surviving the screening and $\vert \bm{M}_\text{scr} \vert$ denote the number of elements in $\bm{M}_\text{scr}$. Then,
$\vert \bm{M}_\text{scr} \vert = \max \left\{20, \vert \bm{M}^\text{top}\vert\right\},$ where $\bm{M}^\text{top}=\left\{\gamma \in \text{nbd}(\gamma): \max\limits_{\gamma \in \text{nbd}(\gamma)}\{\log f(\gamma|y)\} - \log f(\gamma|y) < 6\right\}$ and $\vert \bm{M}^\text{top}\vert$ is number of models in $\bm{M}^\text{top}$. Thus either the models with top 20 highest posterior probabilities or those in $\bm{M}^\text{top}$ are preserved after screening. Then, one of the models in $\bm{M}_\text{scr}$ is drawn according to the corresponding posterior probabilities. It continues to update the current model until certain stopping criterion is satisfied. SSS allows us to move freely among models with different sizes and thus makes it efficient to explore the large model space. However, it's still likely to get entrapped in local maxima of model space. For instance, the MAP model might be in the neighborhood of such a model with a small posterior probability that it is almost unlikely to be drawn. In such cases, the region of the highest posterior model probability would never be visited. To overcome this problem, we borrow the idea from simulated annealing (\citealp{kirk:gela:1983}) and S5 algorithm (\citealp{shin:bhat:2018}), and introduce a temperature parameter in order to broaden the model space explored by the algorithm. This makes a change to the sampling probabilities. Specifically, a model is drawn from the neighborhood with probability proportional to  $f(\gamma|y)^{1/t}$ instead of $f(\gamma|y)$, where $t$ is the temperature.

Our algorithm starts with a complete run of searching with no temperature and uses an ascending temperature schedule to further explore the model space. For each temperature, the starting model is always an empty model. The reason is that the model size tends to grow with increasing temperature. Thus if we take the starting model to be the last model obtained using the previous temperature, the model would become even larger and probably contains a number of unimportant variables. Now let's describe the algorithm in detail. Let $e_i$ be the $i$th $p$ dimensional unit vector, that is, the $i$th element of $\bm{e}_i$ is 1, and all other elements are 0. In the first step for each temperature, we calculate $f(\gamma=\bm{e}_i | \bm{y})$ for $i=1, \ldots, p$ as the the neighbors of an empty model are the ones that contain only one variable. Then a screening of those neighboring models is performed, and a model, $\gamma^{(1)}$, is sampled from $\bm{M}^{(1)}_\text{scr}$ with probability proportional to $f(\gamma|\bm{y})^{1/t}$, where t is the current temperature. In the next step, $f(\gamma|\bm{y})$ is computed for all $\gamma \in \text{nbd}(\gamma^{(1)})$. Again, those neighbors are screened to form $\bm{M}^{(1)}_\text{scr}$ following a random draw from $\bm{M}^{(2)}_\text{scr}$ with probability proportional to $f(\gamma|\bm{y})^{1/t}$. We keep updating the best model so far visited by the algorithm. Clearly, the best model refers to the model with the highest posterior probability. The number of iterations depends on data but generally, from what we have observed, the algorithm hit the MAP model in less than 50 iterations. Although the algorithm is in line with the general shotgun stochastic search algorithm, but it is different from SSS proposed by \citet{hans:dobr:2007} and S5 algorithm by \citet{shin:bhat:2018}, 


\subsection{Rank one Cholesky update}
The highest computation cost of our algorithm is incurred when calculating the posterior probabilities, especially for the adding moves and swapping moves. We use the rank one update to Cholesky factorization to quickly compute all the posteriors of the neighbor models. To describe the method, we again consider 
\begin{align*}
    \log f(\gamma | \bm{y})=& \text { const }+\frac{1}{2}|\gamma| \log \lambda-\frac{1}{2} \log \operatorname{det}\left(X_{\gamma}^{\mathrm{T}} X_{\gamma}+\lambda \mathbf{I}\right) \\ 
    &-\frac{1}{2}(n-1) \log \left\{\mathbf{y}_{C}^{\mathrm{T}} \mathbf{y}_{C}-\mathbf{y}_{C}^{\mathrm{T}} X_{\gamma}\left(X_{\gamma}^{\mathrm{T}} X_{\gamma}+\lambda \mathbf{I}\right)^{-1} \mathbf{X}_{\gamma}^{\mathrm{T}} \mathbf{y}_{C}\right\}, 
\end{align*}
\noindent where $\mathbf{y}_{C}=\mathbf{y}-\bar{y} \mathbf{1}_{n}$ is the vector of centered response values. Suppose we want to compute $f(\bm{\gamma'}|\bm{y})$ given the value of $f(\gamma|\bm{y})$ where $\bm{\gamma'} \in \gamma^{+}$. Without loss of generality, we may assume that $\bm{\gamma'}$ has the $j$th potential predictor variable added to model $\gamma$ and the design matrices corresponding to $\gamma$ and $\bm{\gamma'}$ are $\tilde{X}_{0}$ and $\tilde{X}_{1}=[\tilde{X}_0:x_j]$, where the columns of $\tilde{X}_{0}$ are a permutation of the columns of $X_{\gamma}$ and $x_j$ is the $j$th column of $X$.

Furthermore, we assume that the following two quantities have already been obtained from the previous iteration:
\begin{enumerate}[label=(\arabic*)]
\item
the Cholesky factor of $\tilde{X}_0^{\mathrm{T}} \tilde{X}_0 + \lambda\bm{I}$, that is, we have an upper triangular matrix $\tilde{R}_0$ such that $\tilde{R}_{0}^{\mathrm{T}} \tilde{R}_{0}=\tilde{X}_{0}^{\mathrm{T}} \tilde{X}_{0}+\lambda \mathbf{I}$
\item
the vector $\bm{\tilde{v}}_0$ which satisfies the lower triangular system of equations: $\tilde{R}_{0}^{\mathrm{T}} \bm{\tilde{v}}_0 = \tilde{X}_{0}^{\mathrm{T}} \bm{y}_C$.
\end{enumerate}

Now we want to find an upper triangular matrix
\begin{equation*}
    \tilde{R}_{1}=\left(\begin{array}{cc}{\tilde{R}_{0}} & {\mathbf{s}} \\ {\mathbf{0}^{\mathrm{T}}} & {s_{0}}\end{array}\right)
\end{equation*}
\noindent such that 
\begin{equation*}
    \tilde{R}_{1}^{\mathrm{T}} \tilde{R}_{1}=\tilde{X}_{1}^{\mathrm{T}} \tilde{X}_{1}+\lambda \mathbf{I}=\left(\begin{array}{cc}{\tilde{X}_{0}^{\mathrm{T}} \tilde{X}_{0}+\lambda \mathbf{I}} & {\tilde{X}_{0}^{\mathrm{T}} \mathbf{x}_{j}} \\ {\mathbf{x}_{j}^{\mathrm{T}} \tilde{X}_{0}} & {\mathbf{x}_{j}^{\mathrm{T}} \mathbf{x}_{j}+\lambda}\end{array}\right)
\end{equation*}
\noindent Then we can get $\bm{s}$ and $s_0$ by solving the following linear equations:
\begin{equation}
    \tilde{R}_{0}^{\mathrm{T}} \bm{s} = \tilde{X}_{0}^{\mathrm{T}} \bm{x}_j
\end{equation}

\noindent and $\bm{s}^\mathrm{T}\bm{s} + s^2 = {\mathbf{x}_{j}^{\mathrm{T}} \mathbf{x}_{j}+\lambda}$. Since $\tilde{R}_{0}^{\mathrm{T}}$ is a lower triangular matrix, (6) can be efficiently solved using forward substitution. Once the Cholesky factor $\tilde{R}_{1}$ is found, we can compute the quadratic form in the expression of $\log{f(\gamma'|\bm{y})}$  by observing that 
\begin{itemize}
    \item The quadratic form $\mathbf{y}_{C}^{\mathrm{T}} X_{\gamma}\left(X_{\gamma}^{\mathrm{T}} X_{\gamma}+\lambda \mathbf{I}\right)^{-1} \mathbf{X}_{\gamma}^{\mathrm{T}} \mathbf{y}_{C}$ is equal to $\bm{\tilde{v}}_0^{\mathrm{T}} \bm{\tilde{v}}_0 + u^2$ where $u=\left(\bm{x_j}^{\mathrm{T}}\bm{y}_C - \bm{s}^{\mathrm{T}} \bm{\tilde{v}}_0\right)/s_0$
    
    \item The log-determinant term $\frac{1}{2}|\gamma| \log \lambda-\frac{1}{2} \log \operatorname{det}\left(X_{\gamma}^{\mathrm{T}} X_{\gamma}+\lambda \mathbf{I}\right)$ is equal to $\log \operatorname{det}\tilde{R}_1$ which is also equal to $\log \operatorname{det}\tilde{R}_0 + \log s_0$
\end{itemize}






